World Models with Hints of Large Language Models for Goal Achieving

Reinforcement learning struggles in the face of long-horizon tasks and sparse goals due to the difficulty in manual reward specification. While existing methods address this by adding intrinsic rewards, they may fail to provide meaningful guidance in long-horizon decision-making tasks with large state and action spaces, lacking purposeful exploration. Inspired by human cognition, we propose a new multi-modal model-based RL approach named Dreaming with Large Language Models (DLLM). DLLM integrates the proposed hinting subgoals from the LLMs into the model rollouts to encourage goal discovery and reaching in challenging tasks. By assigning higher intrinsic rewards to samples that align with the hints outlined by the language model during model rollouts, DLLM guides the agent toward meaningful and efficient exploration. Extensive experiments demonstrate that the DLLM outperforms recent methods in various challenging, sparse-reward environments such as HomeGrid, Crafter, and Minecraft by 27.7\%, 21.1\%, and 9.9\%, respectively.

==> icml2024/1_abstract.tex <==
\begin{abstract}

Reinforcement learning struggles in the face of long-horizon tasks and sparse goals due to the difficulty in manual reward specification. While existing methods address this by adding intrinsic rewards, they may fail to provide meaningful guidance in long-horizon decision-making tasks with large state and action spaces, lacking purposeful exploration. Inspired by human cognition, we propose a new multi-modal model-based RL approach named Dreaming with Large Language Models~(DLLM). DLLM integrates the proposed hinting subgoals from the LLMs into the model rollouts to encourage goal discovery and reaching in challenging tasks. By assigning higher intrinsic rewards to samples that align with the hints outlined by the language model during model rollouts, DLLM guides the agent toward meaningful and efficient exploration. Extensive experiments demonstrate that the DLLM outperforms recent methods in various challenging, sparse-reward environments such as HomeGrid, Crafter, and Minecraft by 27.7\%, 21.1\%, and 9.9\%, respectively.

\end{abstract}

%\lzy{However, they fail to establish a clear relationship between intrinsic rewards and corresponding transitions for the agent, hindering the generalization of these intrinsic rewards to more sample-efficient structures, such as Model-Based Reinforcement Learning (MBRL).
% DLLM assigns intrinsic rewards to the agent when the predicted transitions align with the proposed goals (hints) outlined by the language model. Then, DLLM optimizes the combination of extrinsic rewards from the environment and intrinsic rewards from the LLM. 
% Drawing inspiration from human cognition, we propose Dreaming with Large Language Model~(DLLM). This multi-model model-based RL approach learns to use human language to describe the dynamics and integrates hints from the LLM into the model rollouts to improve long-term decision-making. 
%to improve long-term decision-making.
%DLLM leverages human language to describe dynamics by predicting aligned sentence embeddings and integrates the proposed goals (hints) from the LLM into the model rollouts to encourage goal discovery and reaching in challenging tasks.
%to encourage goal discovery and reaching in challenging tasks.
% to improve long-term decision-making.
%\lzy{\sout{model?}} 

==> icml2024/2_intro.tex <==
\section{Introduction}

Reinforcement learning~(RL) is effective when the agents receive rewards that propel them towards desired behaviors~\citep{silver2021reward,ladosz2022exploration}. However, the manual engineering of suitable reward functions presents substantial challenges, especially in complex environments~\cite{xie2023text2reward,dubey2018investigating}. Therefore, solving tasks with long horizons and sparse rewards has long been desired in RL~\cite{Bai_2023, wu2023goal}.

Existing RL methods address this issue by supplementing the extrinsic rewards provided by the environment with an intrinsic reward as an auxiliary objective such as novelty~\citep{burda2019exploration, zhang2019scheduled, zhang2021made}, surprise~\citep{achiam2017surprise}, uncertainty~\citep{bellemare2017distributional, moerland2017efficient, janz2019successor}, and prediction errors~\citep{stadie2015incentivizing, pathak2017curiosity, burda2019large}. 
%However, there are instances where only a few things possess intrinsic factors valuable to the agent's goal, rendering exploration of others meaningless or detrimental to overall performance
Nonetheless, there exist scenarios wherein only a limited set of elements possess inherent factors that are truly valuable to the agent's target objective, rendering the exploration of additional aspects inconsequential or potentially detrimental to the overall system performance~\citep{dubey2018investigating, colas2018gep, du2023guiding}. Some recent researches employ large language models (LLMs) to explore new solutions for this issue~\citep{du2023guiding, zhou2023large, zhang2023adarefiner}. Leveraging prior knowledge from extensive corpus data, these methods aim to encourage the exploration of meaningful states. While these approaches have demonstrated impressive results, they depend on querying the LLM for any unknown environmental conditions, which limits their ability to generalize the acquired language information to other steps. Additionally, due to their model-free nature, these approaches cannot capture the underlying relationships between dynamics and language-based hints. They also fail to leverage planning mechanisms or synthetic data generation to enhance sample efficiency.

\begin{figure*}[h]
% \begin{figure*}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=1\textwidth]{icml2024/pics/algorithm.jpg}}
\caption{The algorithmic overall structure diagram of DLLM, where WM denotes the world model, $o_l$ represents the natural language caption of the observation, $u$ denotes the transition, and $i_k$ corresponds to the intrinsic reward for the $k$-th goal.}
\label{algorithm_big_figure}
\end{center}
\vskip -0.2in
\end{figure*}

To address this issue, we draw inspiration from how humans solve long-horizon tasks efficiently. Humans excel at breaking down overall goals into several sub-goals and strive to plan a reasonable route to accomplish these goals sequentially~\citep{fernando2018learning}. These goals are often associated with specific actions or environmental dynamics and can ideally be expressed in concise natural language. For example, experienced Minecraft players can naturally connect the action ``obtaining iron'' with its prerequisite actions ``find an iron ore'' and ``breaking iron ore''.
% We wonder whether RL agents can acquire such abilities to speed up training and exploration.

Consequently, we propose Dreaming with Large Language Model (DLLM), a multi-modal model-based RL approach that integrates language hints (i.e., goals) from LLMs into the rollouts to encourage goal discovery and reaching in challenging and sparse-reward tasks, as illustrated in Figure \ref{algorithm_big_figure}. DLLM's world model processes visual inputs and sentence embeddings of natural language descriptions for transitions and learns to predict both. It then rewards the agent when the predicted embeddings are close enough to the goal, facilitating the agents' use of inductive bias to achieve task goals. Thanks to the power of prompt-based LLMs, DLLM can influence agents' behaviors in distinct manners based on the prompts provided for identical tasks, resulting in multiple styles of guidance for the agents. For example, when an agent needs to obtain iron in Minecraft, it can be guided directly to break iron ore, explore more for a better policy, or try interpolating both strategies.

Empirically, we evaluate DLLM on various sparse-reward environments, including Homegrid~\citep{lin2023learning}, Crafter~\citep{hafner2022benchmarking}, and Minecraft~\citep{guss2019minerl}. Experimental results demonstrate that DLLM outperforms recent strong methods in task-oriented and exploration-oriented environments, showcasing robust performance in guiding exploration and training of the agent within highly complex scenarios. In Homegrid, Crafter and Minecraft environments, we successfully improve the performance by \textbf{27.7\%}, \textbf{21.1\%} and \textbf{9.9\%}, respectively, compared to the strongest baseline Dynalang~\citep{lin2023learning}, Achievement Distillation~\citep{moon2024discovering}, and DreamerV3~\citep{hafner2023mastering}. We also observe that leveraging more powerful language models and providing the agent with comprehensive language information results in even better performance.

Our contributions are as follows: (a) we propose DLLM, a multi-modal model-based reinforcement learning approach that utilizes human natural language to describe environmental dynamics, and incorporates LLM's guidance in model rollouts to improve the agent's exploration and goal-completion capabilities; (b) based on goals extracted by LLMs, DLLM can generate meaningful intrinsic rewards through an automatic descending mechanism to guide policy learning; (c) experimental results demonstrate that DLLM outperforms recent strong baselines across diverse environments. 

% \begin{figure*}[h]
% % \begin{figure*}[ht]
% % \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=1\textwidth]{icml2024/pics/algorithm.jpg}}
% \caption{The algorithmic overall structure diagram of DLLM, where WM denotes world model, $o_l$ represents the natural language interpretation of the observation, $u$ denotes the transition, and $i_k$ corresponds to the intrinsic reward for the $k$-th goal.}
% \label{algorithm_big_figure}
% \end{center}
% % \vskip -0.2in
% \end{figure*}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.45\linewidth]{icml2024/pics/demo.jpg}
%   \caption{Illustration of our basic idea. It may be hard for the agent to rely on itself to dream rollouts and learn policy in some sparse reward tasks, failing to achieve the desired goal. We introduce the knowledge from the LLM to produce \emph{hints} (a.k.a., goals) and intrinsic rewards to facilitate the training of the agent.}
%   \label{demo}
% \end{figure}
% \ziyu{Yet why would human perform well even on long-horizon and extreme complex tasks? When infant dealing with complex novel situations like walking, they would develop a mental model on how to walk based on both language priors from their parents and visual examples~\citep{forrester1971counterintuitive}. With real experiences on stimulate the mental guidence, they would break down the overall goals into several sub-goals like moving legs forward, and strive to plan a reasonable route to accomplish these goals sequentially~\citep{fernando2018learning} until they tackled the task. Human would learn through the guidence on language format and observations on visual information, we repeat in our head for solutions while updating our cognition for the world through trials. For example, experienced Minecraft players can naturally connect the action ``obtaining iron'' with its prerequisite action \lzy{``find an iron ore'' and} ``breaking iron ore'' based on experience. Can we stimulate this learning process from human cognition to speed up training and exploration, and more importantly to teach the agent better achieving their goals?}
% Thanks to the power of prompt-based LLMs, DLLM can adjust the rewards and affect agents' behaviors according to the prompt for the same tasks, resulting in multiple styles of the trained agents. For example, when an agent needs to obtain iron in Minecraft, it can exploit the current knowledge directly to break iron ore, explore more for a better policy, or try interpolating both strategies.
%\ziyu{To testify whether this framework would assist agents in digital world},
%\lzy{While these approaches have shown impressive results, they rely on querying the LLM for any unknown environmental conditions, lacking the ability to generalize their acquired language information to other steps. Moreover, due to their model-free nature, they cannot capture the relationship between dynamics and language hints, or utilize planning or synthetic data to achieve better sample efficiency, which is the key issue with previous works. (I think this sentence is pretty good!)} %Consequently, the key issue with previous works is their low data efficiency.
%\textcolor{red}{While these approaches have shown impressive results, the auxiliary information they obtain from the LLM is limited by their online iterations. Moreover, they can not capture dynamic information due to their model-free nature.} Consequently, the key issue of previous works is their low data efficiency.
%they often struggle to effectively address long-horizon decision-making problems or capture dynamics information due to their model-free nature. Consequently, they suffer from low data efficiency.}
%\ziyu{While they have shown impressive results}, tasks with long horizons and sparse rewards have long been challenging in RL ~\citep{Bai_2023, wu2023goal} since specifying these reward functions manually requires substantial engineering efforts, especially in complex scenarios~\citep{xie2023text2reward,dubey2018investigating}, Thus, tasks with long horizons and sparse rewards have long been challenging in RL ~\citep{Bai_2023, wu2023goal}. %\ziyu{and embodied environments}.%\ziyu{is such implementation necessary for RL? If not, can we draw some inspiration from pretrained LMs where commonsense knowledge would help the process?}. %Thus, tasks with long horizons and sparse rewards have long been challenging in RL ~\citep{Bai_2023, wu2023goal}\ziyu{and embodied environments}.

%While these approaches have shown impressive results, they rely on querying the LLM for any unknown environmental conditions, lacking the ability to generalize their acquired language information to other steps. Furthermore, owing to their model-free nature, these approaches are unable to capture the underlying relationships between dynamics and language-based hints, nor can they leverage planning mechanisms or synthetic data generation to enhance sample efficiency.

==> icml2024/3_backg.tex <==
\section{Background and Related Work}
\textbf{Model-based RL.} Model-based RL (MBRL) trains a world model through online interactions with the environment to predict rewards and next-step states~\cite{silver2016mastering,silver2017mastering,silver2018general}. With the world model, the agent can plan and optimize its policy from imagined sequences~\cite{hansen2022temporal,lowrey2018plan}. Amidst recent advancements, specific contemporary MBRL methods have acquired a world model that is capable of handling high-dimensional observations and intricate dynamics, achieving notable milestones in various domains~\cite{ha2018world,schrittwieser2020mastering,hafner2019dream,hafner2020mastering,hafner2023mastering,hansen2022temporal}. Akin to our approach, the work of Lin et al.~\cite{lin2023learning} constructs a multimodal world model capable of predicting future visual and textual representations, thereby enabling agents to ground their language generation capabilities within an imagined, simulated environment. We employ the same implementation approach, but further integrate the generated natural language from the LLMs during the planning process into constructing the intrinsic rewards.

\textbf{Intrinsically motivated RL.}
In a sparse-reward environment, agents must take many steps in a decision sequence before receiving a positive reward signal. Collecting practical data for training using only random sampling or noisy RL methods is challenging, especially in complex environments with a large state-action space~\cite{reynolds2002reinforcement, yang2021exploration}. Intrinsically motivated RL is the primary method for addressing sparse reward problems. It provides extra intrinsic dense rewards to the agent, encouraging the agent to explore unvisited areas. Pathak et al.~\cite{pathak2017curiosity} propose using curiosity as an intrinsic reward signal, which measures the agent's proficiency in predicting the consequences of its actions within the latent feature space generated by a self-supervised inverse dynamics model. Burda
et al. propose random network distillation (RND)~\cite{burda2018exploration} that leverages the prediction error of a fixed random neural network on novel states and achieves outstanding results in Montezuma's Revenge. Some subsequent studies improve RND via methods such as distributional modeling~\cite{yang2024exploration}. In addition to the intrinsically motivated method that utilizes state novelty, there are methods for maximizing the diversity of states~\cite{teng2012knowledge, linke2020adapting, wang2023coplanner} and for maximizing the diversity of skills mastered by the agent~\cite{baranes2013active, colas2022autotelic}.

Despite the success of intrinsically motivated RL methods, they may face challenges when dealing with large state-action space and complex task scenarios since they are only encouraged to explore novel states, and not all states are useful for achieving the goal. Purposeless exploration can hinder the performance of the agent. Hence, it is essential to incorporate meaningful encouragement to assist the agent, as highlighted in previous studies~\cite{dubey2018investigating, du2023guiding}. This may involve integrating commonsense knowledge, furnishing explicit subgoals as guides, and employing other relevant strategies to facilitate the agent's learning process. DLLM considers these factors with a specific focus on long-term decision-making. During rollouts, DLLM applies intrinsic rewards when the agent achieves goals set by LLM in previous steps, strengthening the understanding of the agent's contextual connections.

\textbf{Leveraging large language models (LLMs) for language goals.}
Pre-trained LLMs showcase remarkable capabilities, particularly in understanding common human knowledge. Naturally, LLMs can generate meaningful and human-recognizable intrinsic rewards for intelligent agents. Choi et al.~\citep{choi2022lmpriors} leverage pre-trained LLMs as task-specific priors for managing text-based metadata within the context of supervised learning. Kant et al.~\citep{kant2022housekeep} utilize LLMs as commonsense priors for zero-shot planning. Similar efforts are made by Yao
et al., Shinn et al., Wu et al., and Wang et al.,~\cite{yao2022react, shinn2023reflexion, wu2023spring, wang2023voyager}, who propose diverse prompt methods and algorithmic structures to mitigate the problems of hallucination and inaccuracy when employing LLMs directly for decision-making. Carta et al.~\citep{carta2023grounding} examine an approach where an agent utilizes an LLM as a policy that undergoes progressive updates as the agent engages with the environment, employing online reinforcement learning to enhance its performance in achieving objectives. Zhang et al.~\citep{zhang2023bootstrap} 
propose to leverage the LLMs to guide skill chaining. Du
et al. propose ELLM~\citep{du2023guiding}, which leverages LLMs to generate intrinsic rewards for guiding agents, integrating LLM with RL. However, the guidance obtained using this approach is only effective in the short term. DLLM draws inspiration from ELLM and endeavors to extend the guidance from LLMs into long-term decision-making.

%%The Model-Based Reinforcement Learning (MBRL) method involves training a world model through actual interactions with the environment to predict rewards and next-step states. Simultaneously, this world model is used to generate a substantial number of imagined samples for training the policy. Current MBRL methods can learn a world model of high-dimensional observations and complex dynamics and have achieved accomplishments in various domains. DreamerV3 has demonstrated state-of-the-art performance across diverse problem domains, including pixel and state observations and discrete and continuous actions.
% Intrinsically motivated RL has succeeded significantly in sparse reward environments but still faces significant challenges. The main reason is that current methods only encourage the agent to explore a more extensive state space rather than a more meaningful one. Because in an almost infinite state space, purposeless exploration encourages meaningless behavior, while meaningful encouragement (incorporating common sense represented by semantic information) can positively impact the results\cite{dubey2018investigating}.
%% 基本方法提完之后，需要note一下用MBRL做planning for exploration，与这些work的区别， 
%DLLM considers these factors while focusing more on their application in long-term decision-making and introduces the meaningful guidance derived from LLMs into the model rollouts to help implement them effectively over an extended period.%DLLM considers these factors while emphasizing a more profound comprehension of their application in long-term decision-making, delving into a more thorough understanding of how to implement them effectively over an extended period.%DLLM considers these factors and contemplates their application in long-term decision-making.
%\lzy{Curiosity is proposed as an intrinsic reward signal measuring the agent's proficiency in predicting the consequences of its actions within the latent feature space generated by a self-supervised inverse dynamics model~\cite{pathak2017curiosity}. Random network distillation (RND)~\cite{burda2018exploration} leverages the prediction error of a fixed random neural network on novel states and achieves outstanding results in Montezuma's Revenge.}
%into guiding the introduction of intrinsic rewards from the LLM during the planning process. %\lzy{Dynalang}

==> icml2024/4_method.tex <==
\section{Preliminaries}
We consider a partially observable Markov decision process (POMDP) defined by a tuple $(S, A, O, \Omega, P, \gamma, R)$, where $s \in S$ represents the states of the environment, $a \in A$ represents the actions, and observation $o \in \Omega$ is obtained from $O(o|s, a)$. $P(s' | s, a)$ represents the dynamics of the environment, $R$ and $\gamma$ are the reward function and discount factor, respectively. During training, the agent’s goal is to learn a policy $\pi$ that maximizes discounted cumulative rewards, i.e., 
$\max\mathbb{E}_{\pi}\left[\sum_{t=0}^{\infty}\gamma^t R(s_t, a_t)\right].$

Additionally, we define two sets of natural language sentence embeddings: the set of sentence embeddings for transitions, denoted as $U$, and the set of sentence embeddings for goals, denoted as $G$. In this context, each $u \in U$ represents a sentence embedding describing the environmental changes from the previous step to the current step, while $g \in G$ represents a sentence embedding of a goal the LLM intends for the agent to achieve. We permit the LLM to output any content within specified formats, thereby enlarging the support of the goal distribution to encompass the space of natural language strings. Thus, $G$ should encompass all possible $u \in U$, i.e., $U \subset G$.

We also define the goal-conditioned intrinsic reward function $R_{\text{int}}(u|g)$, and the DLLM agent optimizes for an intrinsic reward $R_{\rm int}$ alongside the reward $R$ from the environment. Assuming that goals provided by natural language are diverse, common-sense sensitive, and context-sensitive, we expect that maximizing $R_{\text{int}}$ alongside $R$ ensures that the agent maximizes the general reward function $R$ without getting stuck in local optima.

\section{Dreaming with LLMs}
This section systematically introduces how DLLM obtains guiding information (goals) from LLMs and utilizes them to incentivize the agent to manage long-term decision-making.

\subsection{Goal Generation by Prompting LLMs}
To generate the natural language representations of goals and their corresponding vector embeddings, DLLM utilizes a pretrained SentenceBert model~\cite{reimers2019sentence} and GPT~\cite{ouyang2022training}. For GPT, we use two versions including GPT-3.5-turbo-0315 and GPT-4-32k-0315, which we will refer to as GPT-3.5 and GPT-4 respectively in the following text.

We initially obtain the natural language representation, denoted as $o_l$ ($l$ denotes language, and $o_l$ means natural language description of $o$), corresponding to the information in the agent's current observation $o$. This $o_{l}$ may include details such as the agent's position, inventory, health status, and field of view. We use an observation captioner to obtain the $o_l$ following ELLM~\cite{du2023guiding} (see Appendix~\ref{appendix:captioner} for more details of captioners). Subsequently, we provide $o_l$ and other possible language output from the environment (e.g., the task description in HomeGrid) and the description of environmental mechanisms to LLMs to get a fixed number of goals $g^l_{1:K}$ in the form of natural language, where $K$ is a hyperparameter representing the expected number of goals returned by the LLM. We utilize SentenceBert to convert these goals from natural language into vector embeddings $g_{1:K}$. For different environments, we utilize two specific approaches to obtain goals: 1) having the LLM generate responses for $K$ arbitrary types of goals and 2) instructing the LLM to provide a goal for $K$ specified types (e.g., determining which room to enter and specifying the corresponding action). The second approach is designed to standardize responses from the LLM and ensure that the goals output by the LLM cover all necessary aspects for task completion in complex scenarios.

\subsection{Incorporating Decreased Intrinsic Rewards into Dreaming Processes}
At each online interaction step, we have a transition captioner that gives a language description $u_l$ of the dynamics between the observation and the next observation; the language description $u_l$ is then embedded into a vector embedding $u$. Given the sensory representation $x_0$, language description embedding of transition $u_0$, embeddings of goals $g_{1:K}$, and intrinsic rewards for each goal $i_{1:K}$ of replay inputs, the world model and actor produce a sequence of imagined latent states $\hat{s}_{1:T}$, actions $\hat{a}_{1:T}$, rewards $\hat{r}_{1:T}$, transitions $\hat{u}_{1:T}$ and continuation flags $\hat{c}_{1:T}$, where $T$ represents the total length of model rollouts. We use cosine similarity to measure the matching score $w$ between transitions and goals:
\begin{equation}
\begin{aligned}
w\left(\hat{u} \mid g\right)= \begin{cases}\frac{\hat{u} \cdot g}{\left\|\hat{u}\right\|\|g\|} & \text {if }\frac{\hat{u} \cdot g}{\left\|\hat{u}\right\|\|g\|} >M \\ 0 & \text { otherwise }\end{cases},
\end{aligned}
\end{equation}

where $M$ is a similarity threshold hyperparameter. In this step, we aim to disregard low cosine similarities to some extent, thereby preventing misleading guidance. Moreover, within a sequence, a goal may be triggered multiple times. We aim to avoid assigning intrinsic rewards to the same goal multiple times during a single rollout process, as it could lead the agent to perform simple actions repeatedly and eventually diminish the exploration of more complex behaviors. Hence, we only retain a specific goal's matching score when it first exceeds $M$ in the sequence. The method to calculate the intrinsic reward for step $t$ in one model rollout is written as:
\begin{equation}
\begin{aligned}
r_t^{\text {int}} = \alpha \cdot \sum_{k=1}^{K} w_t^k \cdot i_k \cdot \begin{cases} 1 & \text{if} \ \ t_k^{\prime} \ \ \text{exists} \ \ \text{and} \ \ t = t_k^{\prime} \\ 0 & \text{otherwise} \end{cases}
\end{aligned}
\end{equation}
where $\alpha$ is the hyperparameter that controls the scale of the intrinsic rewards, $t'_k$ represents the time step $t$ when the $w^k_t$ first exceeds $M$ within the range of $1$ to $T$.

Then, we give the method to calculate and decrease $i_{1:K}$. If each goal's reward is constant, the agent will tend to repeat learned skills instead of exploring new ones. We use the novelty measure RND~\citep{burda2018exploration} to generate and reduce the intrinsic rewards from LLMs, which effectively mitigates the issue of repetitive completion of simple tasks. To be more specific, after sampling a batch from the replay buffer, we extract the sentence embeddings of the goals from them: $g_{1:B,1:L,1:K}$, where $B$ is the batch size, and $L$ is the batch length. Given the target network $f:G\rightarrow{\mathbb{R}}$ and the predictor neural network $\hat{f_\theta}:G\rightarrow{\mathbb{R}}$, we calculate the prediction error:
\begin{equation}
\begin{aligned}
e_{1:B,1:L,1:K}=\|\hat{f}_{\theta}(g)-f(g)\|^2.
\end{aligned}
\end{equation}
Subsequently, we update the predictor neural network and the running estimates of reward standard deviation, then standardize the intrinsic reward:
\begin{equation}
\begin{aligned}
i_{1:B,1:L,1:K}=(e_{1:B,1:L,1:K}-m)/{\sigma},
\end{aligned}
\end{equation}
where $m$ and $\sigma$ stand for the running estimates of the mean and standard deviation of the intrinsic returns.

\subsection{World Model and Actor Critic Learning}

We implement the world model with Recurrent State-Space Model (RSSM)~\cite{hafner2019learning}, with an encoder that maps sensory inputs $x_t$ (e.g., image frame or language) and $u_{t}$ to stochastic representations $z_t$. Afterward, $z_t$ is combined with past action $a_t$ and recurrent state $h_t$ and fed into a sequence model, denoted as ``seq'', to predict $\hat{z}_{t+1}$:
\begin{equation}
\begin{aligned}
\hat{z}_t, h_t=\operatorname{seq}\left(z_{t-1}, h_{t-1}, a_{t-1}\right),
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
z_t \sim \operatorname{encoder}\left(x_t, u_t, h_t\right),
%\hat{x}_t, \hat{u}_{t}, \hat{r}_t, \hat{c}_t=\operatorname{dec}\left(z_t, h_t\right),
\end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
\hat{x}_t, \hat{u}_{t}, \hat{r}_t, \hat{c}_t=\operatorname{decoder}\left(z_t, h_t\right),
\end{aligned}
\end{equation}
where $\hat{z_t}$, $\hat{x}_t$, $\hat{u}_{t}$, $\hat{r}_t$, $\hat{c}_t$ denotes the world model prediction for the stochastic representation, sensory representation, transition, reward, and the episode continuation flag. The encoder and decoder employ convolutional neural networks (CNN) for image inputs and multi-layer perceptrons (MLP) for other low-dimensional inputs. After obtaining multi-modal representations from the decoder and sequence model, we employ the following objective to train the entire world model in an end-to-end manner:
\begin{equation}
\begin{aligned}
\mathcal{L}_{\rm total}={\mathcal{L}_x}+\mathcal{L}_{u}+\mathcal{L}_r+\mathcal{L}_{c}+{\beta_1}\mathcal{L}_{\rm pred}+{\beta_2}\mathcal{L}_{\rm reg},
\end{aligned}
\end{equation}
in which $\beta_1=0.5$, $\beta_2=0.1$, and all sub loss term are written as:
\begin{equation}
\begin{aligned}
&\text{Sensation Loss:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2, \\
&\text{Transition Loss:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right), \\
&\text{Reward Loss:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right), \\
&\text{Continue Loss:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right), \\
&\text{Prediction Loss:} &&\mathcal{L}_{\text{pred}}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}\left(z_t\right) \| \hat{z}_t\right]\right), \\
&\text{Regularizer:} &&\mathcal{L}_{\text{reg}}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}\left(\hat{z}_t\right)\right]\right),
\end{aligned}
\end{equation}

where $\rm catxent$ is the categorical cross-entropy loss, $\rm binxent$ is the binary cross-entropy loss, $\rm sg$ is the stop gradient operator, KL refers to the Kullback-Leibler (KL) divergence. Details of the $\text{twohot}(\cdot)$ can be found in Appendix \ref{appendix:twohot}.

We adopt the widely used actor-critic architecture for learning policies, where the actor executes actions and collects samples in the environment while the critic evaluates whether the executed action is good. We denote the model state as $s_t = concat(z_t,h_t)$. The actor and the critic give:
\begin{equation}
\begin{aligned}
&\text{Actor: } &&\pi_\theta(a_t \mid s_t), &&\quad &\text{Critic: } && V_\psi(s_t).
\end{aligned}
\end{equation}
Note that both the actor network and the critic network are simple MLPs. The actor aims to maximize the cumulative returns with the involvement of intrinsic reward, i.e.,
\begin{equation}
\begin{aligned}
R_t \doteq \sum_{\tau=0}^{\infty} \gamma^\tau (r_{t+\tau}+r^{\rm int}_{t+\tau}).
\end{aligned}
\end{equation}
The intrinsic rewards beyond the prediction horizon $T$ are inaccessible, and we set them to zero. The details of bootstrapped $\lambda$-returns ~\cite{sutton2018reinforcement}. Then the bootstrapped $\lambda$-returns ~\cite{sutton2018reinforcement} could be written as:
\begin{equation}
\begin{aligned}
R_t^\lambda \doteq r_t+\gamma c_t\left((1-\lambda) V_\psi\left(s_{t+1}\right)+\lambda R_{t+1}^\lambda\right), &&\quad R_T^\lambda \doteq V_\psi\left(s_T\right).
\end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% R_T^\lambda \doteq V_\psi\left(s_T\right).
% \end{aligned}
\end{equation}

The actor and the critic are updated via the following losses:
\begin{equation}
\begin{aligned}
& \mathcal{L}_V=\operatorname{catxent}\left(V_\psi(s_t), \operatorname{sg}\left(\operatorname{twohot}\left(R_t\right)\right)\right), \\
& \mathcal{L}_\pi=-\frac{\operatorname{sg}\left(R_t-V(s_t)\right)}{\max (1, S)} \log \pi_\theta\left(a_t \mid s_t\right)-\eta \mathrm{H}\left[\pi_\theta\left(a_t \mid s_t \right)\right].
\end{aligned}
\end{equation}

where $S$ is the exponential moving average between the 5th and 95th percentile of $R_t$. We summarize the detailed pseudocode for DLLM in Appendix~\ref{appendix:psecode}. %\lzy{(Is it better for us, to move these to appendix and cite RSSM, then use the space to write the detailed analysis?).}

% where $S$ = ema(Per($R_t$, 95) - Per($R_t$, 5)) is used for trading off the two actor loss terms without having to tune hyperparameters, where ema is the exponential moving average~\cite{hilton2022batch}, and Per means percentile. A summary of DLLM is in Appendix~\ref{appendix:psecode}.

%which is the same in DreamerV3.

%Depending on the environment, we choose distinct goal spaces $G$, each representing the set of goals that the Large Language Model (LLM) can provide. Moreover, the DLLM agent optimize for an intrinsic reward $R_{int}$ alongside the reward $R$ from the environment. 
% $$
% {R_{int\_final}}_{1:T}=max_k({R_{int\_first}}^k_{1:T}).
% $$
% Then we use the intrinsic reward derived from RND 
% Then we include intrinsic rewards for accomplishing goals. During the process, we first compute the reward for a given goal $g$ by computing the semantic similarity between the transition and the goal generated by LLM, where the semantic similarity is the cosine similarity of representations of goals and their vector embedding from the Language Model's encoder. 
% % 公式，这里是计算reward的公式，需要把ELLM里面的这个部分改成一个公式 %
% In our model, we include a masked language model SentenceBert as our language model. Then we assess the cosine similarity between the goal vectors and transition tokens, by computing dot products and norms of the vectors and then calculating their cosine similarity. After we select the maximum cosine similarity for each 16 dreaming steps in each trajectory. We apply a mask to retain only the maximum similarity values as the chosen one and setting the others to zero. Additionally, similarities below a specific threshold are also zeroed out. This adjusted similarity is multiplied by the goal intrinsic reward to obtain a modified intrinsic reward for each goal. Finally, the overall intrinsic reward is updated by taking the maximum value between the newly calculated reward and the current intrinsic reward for each element.
%We choose cosine similarity to measure alignment between atomic agent actions and freeform LLM generations. When the caption of a transition is sufficiently close to the goal description (∆ > T ), where T is a similarity threshold hyperparameter, the agent is rewarded proportionally to their similarity. 
% As a result, the general reward function of methods can be rewritten:
% We include intrinsic rewards to explore outcomes rather than actions.
% We issue inquiries to the large language model in a predetermined format. This process results in obtaining a fixed number of natural language expressions for the sub-goals 
% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{icml2024/pics/world_model_zhanwei.png}}
% \caption{World Model and its description}
% \label{world_model}
% \end{center}
% \vskip -0.2in
% \end{figure}
% We basically adopt the same training approach for the Actor and Critic as DreamerV3. The actor and critic networks purely learn from the sequence dreamed from the world model. Model state is defined as the concatenation of the $z_t$ and $h_t$: $s_t \doteq\left\{h_t, z_t\right\}$ here. Actor and Critic networks both are MLPs:
% The implementation of RND involves a straightforward batch RND approach. After sampling a batch from the replay buffer, we input the goal portion of the batch into the batch RND network and obtain the intrinsic reward for each corresponding goal.
% Additionally, we define two sets of natural language sentence embedding: the set of transitions’ sentence embeddings $L$ and the set of goals‘ sentence embedding $G$. Here, each $l \in L$ is a sentence embedding of language description of the change that happened in the environment from the previous step to the current step, while $g \in G$ represents a sentence embedding of a goal that the large language model aims for the agent to accomplish. We stipulate that goals are always achievable, i.e., $G \subset L$.
%describes the changes in the environment and the agent from the previous step to the current step, 
% Under POMDP, according to our algorthms's nature of language inputs, we define two sets under natural language background: the environmental transitions set $TRAN$ and the goal set $G$. Here, $tran \in TRAN$ describes changes from the previous step to the current step in both the environment and the agent, while $goal \in G$ represents the objectives that the large language model guided the agent to accomplish. 
%  In this setting, We assume all the goals are always achievable, i.e., $G \subset TRAN$. We define the goal-conditioned intrinsic reward function $R_{\text{int}}(tran|g)$, and DLLM agent optimize for an intrinsic reward $R_{int}$ alongside the reward $R$ from the environment. We assume that goals provided by natural language are inherently diverse, common-sense sensitive, and context-sensitive. Therefore, maximizing $R_{\text{int}}$ alongside $R$ ensures that the agent maximizes general reward function $R$ without getting stuck in local optima.
% Given the visual presentation $x_1$, transition $tran_1$, goals $g^{1:K}$, and intrinsic rewards for each goal ${{r}^{int}_g}_{1:K}$ of replay inputs, the world model and actor produce a sequence of imagined model states $s_{1:T}$, actions $a_{1:T}$, rewards $r_{1:T}$, transitions $tran_{1:T}$ and continuation flags $c_{1:T}$. We use cosine similarity to measure the match between transitions and goals:
% Where $M$ is a similarity threshold hyperparameter. Subsequently, we can obtain the match score ${match}^{1:K}_{1:T}$ between each transition and each goal in this sequence batch.
% Within a sequence, a goal may be triggered multiple times. We aim to avoid assigning intrinsic rewards to the same goal multiple times during a single dreaming process, as it could potentially lead the agent to repeatedly perform simple actions, thereby diminishing the exploration of more complex behaviors. Therefore, within the same sequence, for a specific goal, we only retain its match score when it is firstly higher than $M$:
% We initially obtain the natural language representation, denoted as $C(o)$, corresponding to the information contained in the agent's current observation $o$, where $C: O \rightarrow \Sigma$ is a captioner that translates the abstract observation representation it receives into natural language. This may include details such as the agent's position, carried objects, agent's status, and visible objects. Unless explicitly designed otherwise, we do not incorporate any information beyond the current observation in the environment. 
% In detail, after sampling a batch from the replay buffer, we extract the goal embeddings part from them: $g_{1:B,1:L,1:K}$. Given the target network $f:E\rightarrow{\mathbb{R}}$ and the predictor neural network $\hat{f_\theta}:E\rightarrow{\mathbb{R}}$, we calculate the prediction error $i_{1:B,1:L,1:K}=\|\hat{f}_{\theta}(g)-f(g)\|^2$, update the predictor neural network, update running estimate of reward standard deviation and normalize the intrinsic reward:
% As the reinforcement learning agent progresses through training, it gradually acquires skills that are incentivized by additional rewards. However, if these rewards remain constant, we found the agent tends to repeatedly perform learned skills without exploring those it hasn't mastered yet. Therefore, we employ an RND network to provide intrinsic rewards for each transition, and we reduce this intrinsic reward in tandem with the updates to the RND network. This approach effectively mitigates the issue of repetitive completion of simple tasks.
% The encoder and decoder employ convolutional neural networks (CNN) for image inputs and multi-layer perceptrons (MLP) for other low-dimensional inputs. After obtaining multimodal representations from the decoder and sequence model, we employ the following objective to train the entire World Model in an end-to-end manner:
% Subsequently, we provide $C(o)$, $G$ and other necessary information such as current task and descriptions of environmental mechanisms to LLMs, to get a fixed number of goals $g_{1:K}$ in the form of natural language, where K is a hyperparameter. We utilize SentenceBert to convert these sub-goals from natural language into vector embeddings $e(g)_{1:K}$. For distinct environments, we utilize two specific approaches to obtain goals: (1) having the large language model generate responses for K arbitrary types of goals, and (2) instructing the large language model to provide a goal for K specified types (e.g., determining which room to enter and specifying the corresponding action).
%In order to verify whether the agent accomplishes the goals suggested by GPT during the dreaming process, we implemented a transition captioner: $C_{\text{transition}}: O \times A \times O \rightarrow \Sigma$.
% The structure of our world model is illustrated in Figure \ref{world_model}. We implemented the world model using the structure of the Recurrent State-Space Model (RSSM). We utilize an encoder to map sensory inputs $x_t$ and $tran_{t}$ to stochastic representations $z_t$. Subsequently, $z_t$ is combined with past action $a_t$ and recurrent state $h_t$ and fed into a sequence model to predict $\hat{z}_{t+1}$:
%(GPT ~\cite{ouyang2022training}) (SentenceBert) 

%where $t'_k$ represents the time step $t$ when the cumulative sum $w^k_{1:T}$ first exceeds $M$ within the range of $1$ to $T$. $\mathbbm{1}(\cdot)$ is the indicator function, and $\alpha$ is a hyperparameter that controls the scale of the intrinsic rewards.

% \lzy{\sout{If the similarity between a transition and multiple goals exceeds the threshold $M$, we only consider the goal with the highest similarity:}
% \begin{equation}
% \begin{aligned}
% \text{index}_t = \begin{cases} \text{None}, & \text{if all }p^{1:K}_t \text{are zero}, \\ \arg\max_k p^k_t, & \text{otherwise.}\end{cases}
% \end{aligned}
% \end{equation}
% }

% Then, we calculate the final intrinsic reward:
% \begin{equation}
% \begin{aligned}
% r^{int}_{t}=\begin{cases}{\alpha}\cdot{i_{{\text{index}}_t}}, & \text{if index}_t\text{ is not None,} \\ 0, & \text{otherwsie,} \end{cases}
% \end{aligned}
% \end{equation}
%where $\alpha$ is a hyperparameter that controls the scale of the intrinsic rewards.

% We adopt the same training approach for the Actor and Critic as DreamerV3 ~\cite{hafner2023mastering}. The actor and critic networks purely learn from the sequence dreamed from the world model. Model state is defined as the concatenation of the $z_t$ and $h_t$: $s_t \doteq\left\{h_t, z_t\right\}$ here. Actor and Critic networks both are MLPs:

% \usepackage{multicol}
% \begin{multicols}{4}
% \begin{align}
% &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2, \\
% &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, u_t\right), \\
% &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}(r_t)\right), \\
% &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right), \\
% &\text{Prediction:} &&\mathcal{L}_{\text{pred}}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}(z_t) \| \hat{z}_t\right]\right), \\
% &\text{Regularizer:} &&\mathcal{L}_{\text{reg}}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}(\hat{z}_t)\right]\right).
% \end{align}
% \end{multicols}}

% \begin{aligned}
% &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2, \quad
% &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right),\\
% &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right), \quad
% &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),\\
% &\text{Prediction:} &&\mathcal{L}_{\text {pred }}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}\left(z_t\right) \| \hat{z}_t\right]\right), \quad
% &\text{Regularizer:} &&\mathcal{L}_{\text {reg }}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}\left(\hat{z}_t\right)\right]\right).
% \end{aligned}
% \begin{flaligned}
%    \left{
%    &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2,
%    } 
%    \right{
%    &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right)
%    }
   % \left{
   % &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right),}
   % \right{
   %  &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),}
   %  }
% \end{flaligned}
% \begin{flaligned}
%     \left{
%    &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right),}
%    \right{
%     &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),}
% \end{flaligned}

% \begin{aligned}
% &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2,
% &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right),\\
% &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right),
% &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),\\
% &\text{Prediction:} &&\mathcal{L}_{\text {pred }}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}\left(z_t\right) \| \hat{z}_t\right]\right),
% &\text{Regularizer:} &&\mathcal{L}_{\text {reg }}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}\left(\hat{z}_t\right)\right]\right).
% \end{aligned}
% \begin{aligned}
% &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2,
% &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right),\\
% &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right),
% &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),\\
% &\text{Prediction:} &&\mathcal{L}_{\text {pred }}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}\left(z_t\right) \| \hat{z}_t\right]\right),
% &\text{Regularizer:} &&\mathcal{L}_{\text {reg }}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}\left(\hat{z}_t\right)\right]\right).
% \end{aligned}
% \end{equation*}}

%we directly modify the original environment to always output an $o_l$ that accurately describes the current observation $o$. This process can be considered as having a perfect observation captioner that is capable of transforming image observations into natural language descriptions in a completely accurate manner. In our experiments, we do not focus on the training of such a captioner. Meanwhile, unless explicitly designed otherwise, we strictly do not incorporate any information beyond the current observation in the environment.

% Subsequently, we can obtain the matching score $w^{1:K}_{1:T}$ between each transition and each goal in this sequence batch.

% ~\lzy{(I wonder if this is the right location to give definition for transition captioner?)}

 %Prompt LLMs to Generate Goals
% Similar to ELLM ~\cite{du2023guiding}, 
% DLLM utilizes the goals' natural language representations and their corresponding vector embeddings. 
% DLLM employs GPT~\cite{ouyang2022training} and a pretrained SentenceBert model~\cite{reimers2019sentence} to generate the goals' natural language representations and their corresponding vector embeddings. 

%\sout{Assuming that goals provided by natural language are diverse, common-sense sensitive, and context sensitive, we expect maximizing $R_{\text{int}}$ alongside $R$ ensures that the agent maximizes general reward function $R$ without getting stuck in local optima.}

%$\mathbbm{1}(\cdot)$ is the indicator function,

% \begin{equation}
% \begin{aligned}
% r_t^{\text {int} }=\alpha \cdot \sum_{k=1}^{K} w_t^k \cdot i_k \cdot \mathbbm{1}\left(t=t_k^{\prime}\right),
% \end{aligned}
% \end{equation}

% &\text{Image:} &&\mathcal{L}_x=\left\|\hat{x}_t-x_t\right\|_2^2,
% &\text{Transition:} &&\mathcal{L}_{u}=\operatorname{catxent}\left(\hat{u}_t, {u}_t\right),\\
% &\text{Reward:} &&\mathcal{L}_r=\operatorname{catxent}\left(\hat{r}_t, \operatorname{twohot}\left(r_t\right)\right),
% &\text{Continue:} &&\mathcal{L}_c=\operatorname{binxent}\left(\hat{c}_t, c_t\right),\\
% &\text{Prediction:} &&\mathcal{L}_{\text {pred }}=\max \left(1, \operatorname{KL}\left[\operatorname{sg}\left(z_t\right) \| \hat{z}_t\right]\right),
% &\text{Regularizer:} &&\mathcal{L}_{\text {reg }}=\max \left(1, \operatorname{KL}\left[z_t \| \operatorname{sg}\left(\hat{z}_t\right)\right]\right),

% The intrinsic reward beyond the prediction horizon T=16 is inaccessible, so we don't consider this part. 

% The complete loss of the actor-critic algorithm and other details can be described as:

% \begin{aligned}
% &\text{Actor: } &&\pi_\theta\left(a_t \mid s_t\right)
% &\text{Critic: } && V_\psi(s_t)
% \end{aligned}

%~\sout{However, if the reward for each goal remains constant, we find that the agent tends to repeatedly perform learned skills instead of exploring those it has not mastered yet.} %To address this issue, we reduce the intrinsic rewards from LLMs when the skills are repeatedly suggested by using novelty measures such as RND~\cite{burda2018exploration}.

%\subsection{Applying Intrinsic Rewards in Dreaming}

% \subsection{\lzy{Decreasing Intrinsic Rewards Applied in Dreaming}}
% As the agent evolves during training, it acquires skills incentivized by additional rewards. \lzy{However, if each goal's reward is constant, the agent will tend to repeat learned skills instead of exploring new ones. To address this issue, we use the novelty measure RND~\citep{burda2018exploration} to generate and reduce the intrinsic rewards from LLMs when skills are repeatedly suggested.} We find this approach effectively mitigates the issue of repetitive completion of simple tasks.

% \lzy{To be more specific}, after sampling a batch from the replay buffer, \lzy{we extract the sentence embeddings of the goals from them: $g_{1:B,1:L,1:K}$,} where $B$ is the batch size, and $L$ is the batch length. Given the target network $f:G\rightarrow{\mathbb{R}}$ and the predictor neural network $\hat{f_\theta}:G\rightarrow{\mathbb{R}}$, we calculate the prediction error:
% \begin{equation}
% \begin{aligned}
% e_{1:B,1:L,1:K}=\|\hat{f}_{\theta}(g)-f(g)\|^2.
% \end{aligned}
% \end{equation}
% Subsequently, we update the predictor neural network and the running estimates of reward standard deviation, then standardize the intrinsic reward:
% \begin{equation}
% \begin{aligned}
% i_{1:B,1:L,1:K}=(e_{1:B,1:L,1:K}-m)/{\sigma},
% \end{aligned}
% \end{equation}
% where $m$ and $\sigma$ stand for the running estimates of the mean and standard deviation of the intrinsic returns.

% At each online interaction step, we have a transition captioner that gives a language description $u_l$ of the dynamics between the observation and the next observation; the language description $u_l$ is then embedded in a vector embedding $u$. Given the visual representation $x_0$, language description embedding of transition $u_0$, embeddings of goals $g_{1:K}$, and intrinsic rewards for each goal $i_{1:K}$ of replay inputs, the world model and actor produce a sequence of imagined latent states $\hat{s}_{1:T}$, actions $\hat{a}_{1:T}$, rewards $\hat{r}_{1:T}$, transitions $\hat{u}_{1:T}$ and continuation flags $\hat{c}_{1:T}$, where $T$ represents the total length of model rollouts. We use cosine similarity to measure the matching score $w$ between transitions and goals:
% \begin{equation}
% \begin{aligned}
% w\left(\hat{u} \mid g\right)= \begin{cases}\frac{\hat{u} \cdot g}{\left\|\hat{u}\right\|\|g\|} & \text {if }\frac{\hat{u} \cdot g}{\left\|\hat{u}\right\|\|g\|} >M \\ 0 & \text { otherwise }\end{cases},
% \end{aligned}
% \end{equation}

% where $M$ is a similarity threshold hyperparameter. In this step, we aim to disregard low cosine similarities to some extent, thereby preventing misleading guidance. Moreover, within a sequence, a goal may be triggered multiple times. We aim to avoid assigning intrinsic rewards to the same goal multiple times during a single rollout process, as it could potentially lead the agent to repeatedly perform simple actions, and eventually diminish the exploration of more complex behaviors. Hence, for a specific goal, we only retain its matching score when it first exceeds $M$ in the sequence. The method to calculate the intrinsic reward for step $t$ in one model rollout is finally written as:
% \begin{equation}
% \begin{aligned}
% r_t^{\text {int}} = \alpha \cdot \sum_{k=1}^{K} w_t^k \cdot i_k \cdot \begin{cases} 1 & \text{if} \ \ t_k^{\prime} \ \ \text{exists} \ \ \text{and} \ \ t = t_k^{\prime} \\ 0 & \text{otherwise} \end{cases}
% \end{aligned}
% \end{equation}
% where $\alpha$ is the hyperparameter that controls the scale of the intrinsic rewards, $t'_k$ represents the time step $t$ when the $w^k_t$ first exceeds $M$ within the range of $1$ to $T$.

==> icml2024/5_experiments.tex <==
\section{Experiments}

The primary goal of our experiments is to substantiate the following claim: DLLM helps the agent by leveraging the guidance from the LLM during the dreaming process, thereby achieving improved performance in tasks. Specifically, our experiments test the following hypotheses:
\begin{itemize}
\item \textbf{(H1)} Through proper prompting, DLLM can comprehend complex environments and generate accurate instructions to assist intelligent agents in multi-task environments.
\item \textbf{(H2)} DLLM can leverage the generative capabilities of LLMs to obtain reasonable and novel hints, aiding agents in exploration within challenging environments.
\item \textbf{(H3)} DLLM can significantly accelerate the exploration and training of agents in highly complex, large-scale, near-real environments that necessitate rational high-dimensional planning.
\item \textbf{(H4)} DLLM can be more powerful when leveraging stronger LLMs or receiving additional language information.
\end{itemize}

\textbf{Baselines.} Since we include natural language information in our experiments, we consider employing ELLM~\cite{du2023guiding} and Dynalang~\cite{lin2023learning} as baselines.\footnote{For ELLM and Dynalang, we utilize their official implementations for experimentation. For ELLM, we prompt the LLM and obtain goals following the same procedure as in our method. All language information, including the goals obtained from the LLMs, is encoded into sentence embeddings to feed Dynalang.} We also compare against other recent strong baseline algorithms that do not utilize natural language in each environment.%We refer to this modified version of Dynalang as Dynalang (w/ goals).

\textbf{Environments.} We conduct experiments on three environments: HomeGrid~\cite{lin2023learning}, Crafter~\cite{hafner2022benchmarking}, and Minecraft based on MineRL~\cite{guss2019minerl}. These environments span first-person to third-person perspectives, 2D or 3D views, and various types and levels of task complexity.

\textbf{Captioner and Language Encodings.} Within each environment, we deploy an observation captioner and a transition captioner to caption observations and transitions, respectively. Transition captions are stored in the replay buffer for the agent's predictive learning, while observation captions provide pertinent information for LLM. For language encoding, we employ SentenceBert \emph{all-MiniLM-L6-v2}~\cite{wang2020minilm} to convert all natural language inputs into embeddings.

\textbf{The Quality of Generated Goals.} To measure the quality of goals generated by LLMs during online interaction in the environment, we selected the following metrics: novelty, correctness, context sensitivity, and common-sense sensitivity. See the detailed explanations and experiments in Appendix~\ref{appendix:criterias}.

\textbf{Cache.} As each query to the LLM consists of an object-receptacle combination, we implement a cache for each experiment to efficiently reuse queries, thereby reducing both time and monetary cost.

\subsection{HomeGrid}

\textbf{Environment description.} HomeGrid is a multi-task reinforcement learning environment structured as a grid world, where agents get partial pixel observations and language hints (e.g., the descriptions of tasks). We reduce the map size to {10$\times$10} to expedite the overall training of the agent and incorporate icon signals to indicate actions for opening bins. For each step, we have the captioners to caption the observation and transition. The other components of the environment remain unchanged. More details can be seen in Appendix~\ref{appendix:homegridmod}.

To support our claims, we design various settings where the environment provides different levels of information along with distinct language hints for each, as outlined in Table \ref{tab:environment_settings}, to help address hypothesis \textbf{H4}.
\begin{table}[ht]
\centering
\caption{Description of different environment settings}
\begin{tabular}{lp{11.8cm}}
\toprule
\textbf{Setting} & \textbf{Description} \\
\midrule
Standard & The environment provides task descriptions in natural language form. \\
Key info & The environment additionally provides task-relevant objects' location and status information. \\
Full info & The environment additionally provides the location and status information of all objects on the map. For bins, the correct opening actions will also be instructed. \\
Oracle & The agent will always receive accurate instructions. \\
\bottomrule
\end{tabular}
\label{tab:environment_settings}
\end{table}

\textbf{Query prompts, LLM choices, and Goals Generated.} Each query prompt consists of the caption of the agent's current observation and a request for the LLM to generate a goal for each of the two types: ``where to go'' and ``what to do'', respectively. For full prompts and examples, please see Appendix~\ref{appendix:homegridprompt}. We select GPT-4 as the base LLM for all experiments in HomeGrid. Queries to the GPT are made every ten steps. We test the quality of the goals generated in the Appendix~\ref{appendix:homegrid_goals_analysis}.

%\begin{figure}[ht]
\begin{wrapfigure}{r}{0.55\textwidth}
\centering
\includegraphics[width=0.55\textwidth]{icml2024/pics/homegrid_plot.pdf}
%\includegraphics[width=0.5\columnwidth]{icml2024/pics/homegrid_mini_10M.pdf}
%\vspace{-3mm}
\caption{HomeGrid experiments results. Curves averaged over 5 seeds with shading representing one-eighth of the standard deviation.}
\label{homegrid}
\vspace{-2mm}
\end{wrapfigure}
%\end{figure}

\textbf{Performance.} The overall results are depicted in Figure \ref{homegrid}. The baseline algorithm ELLM fails in HomeGrid, likely because it struggles to comprehend the sentence embeddings required to describe the task. Our method outperforms baseline algorithms utilizing the same information in the standard setting, showing strong evidence for \textbf{H1} and \textbf{H3}. Moreover, in the Key info, Full info, and Oracle settings, DLLM demonstrates enhanced performance with increasing information. In the overall context of reduced error prompts in the Full info, DLLM consistently demonstrates a more pronounced advantage throughout the training period. The results of the Full info and Oracle settings show no significant difference. These findings support hypothesis \textbf{H4}.

\subsection{Crafter}

\begin{figure}[ht]
    \centering
    \subfigure[]{
    \includegraphics[width=0.40\linewidth]{icml2024/pics/spr_overall.pdf}
    \label{fig:crafter_sub_spr}
    }\hspace{0mm}
  \subfigure[]{
    \includegraphics[width=0.56\linewidth]{icml2024/pics/1M_successes.pdf}
    \label{fig:crafter_sub_successes}
  }
  \caption{\textbf{Left.} The bar chart comparison of the means and standard deviations between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin. \textbf{Right}. The logarithmic scale success rates for unlocking 18 in 22 achievements at 1M (with the remaining four never achieved otherwise). DLLM surpasses baselines in most achievements, particularly excelling in challenging tasks such as ``make stone pickaxe/sword'' and ``collect iron''. ``AD'' refers to Achievement Distillation~\cite{moon2024discovering}, we utilize its official code base to obtain success rate results.}%We conducted experiments using its official code base to obtain success rate results.
  \label{crafter_sqr}
  \vspace{-4mm}
\end{figure}

\textbf{Environment description.} The Crafter environment is a grid world that features top-down graphics and discrete action space. Crafter is designed similarly to a 2D Minecraft, featuring a 
procedurally generated, partially observable world where players can collect or craft a variety of artifacts. In Crafter, the player's goal is to unlock the entire achievement tree, which consists of 22 achievements. As the map is designed with entities capable of harming the player (e.g., zombies, skeletons), the player must also create weapons or place barriers to ensure survival.

\textbf{Extra baselines.} We compared three additional types of baselines that do not utilize language information: (1) LLM-based solutions: SPRING~\cite{wu2023spring}, Reflexion~\cite{shinn2023reflexion}, ReAct~\cite{yao2022react}, standalone GPT-4 (step-by-step instructions), (2) model-based RL baseline: DreamerV3~\cite{hafner2023mastering}, (3) model-free methods: Achievement Distillation~\cite{moon2024discovering}, PPO~\cite{schulman2017proximal}, Rainbow~\cite{hessel2017rainbow}. We also add human experts~\cite{hafner2022benchmarking} and random policy as additional references.
%(4) intrinsical methods: RND~\cite{burda2019exploration}, Plan2Explore\cite{sekar2020planning}.

\textbf{Query prompts, LLM choices, and Goals Generated.} Each query prompt contains the caption of the agent's current observation description and a request to have the LLM generate five goals. In this portion, we conduct evaluations using two popular LLMs, GPT-3.5 and GPT-4. Through these assessments, we explore whether a more robust LLM contributes to enhanced agent performance, addressing hypothesis \textbf{H4}. Queries to the GPT are made every ten steps. We test the quality of the goals generated in the Appendix~\ref{appendix:crafter_goals_analysis}.

\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \vspace{-4mm}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
      \hline
      Method & Score & Reward & Steps \\
      \hline
      DLLM (w/ GPT-4) & \textbf{38.1}$\pm$1.2 & 15.4$\pm$1.1 & 5M \\
      DLLM (w/ GPT-3.5) & \textbf{37.6}$\pm$1.6 & 14.5$\pm$1.5 & 5M \\
      AdaRefiner (w/ GPT-4) & 28.2$\pm$1.8 & 12.9$\pm$1.2 & 5M \\
      AdaRefiner (w/ GPT-3.5) & 23.4$\pm$2.2 & 11.8$\pm$1.7 & 5M \\
      ELLM & - & 6.0$\pm$0.4 & 5M \\
      \hline
      DLLM (w/ GPT-4) & \textbf{26.4}$\pm$1.3 & 12.4$\pm$1.3 & 1M \\
      DLLM (w/ GPT-3.5) & \textbf{24.4}$\pm$1.8 & 12.2$\pm$1.6 & 1M \\
      Achievement Distillation & 21.8$\pm$1.4 & 12.6$\pm$0.3 & 1M \\
      Dynalang & 16.4$\pm$1.7 & 11.5$\pm$1.4 & 1M \\
      AdaRefiner (w/ GPT-4) & 15.8$\pm$1.4 & 12.3$\pm$1.3 & 1M \\
      PPO (ResNet) & 15.6$\pm$1.6 & 10.3$\pm$0.5 & 1M \\
      DreamerV3 & 14.5$\pm$1.6 & 11.7$\pm$1.9 & 1M \\
      PPO & 4.6$\pm$0.3 & 4.2$\pm$1.2 & 1M \\
      Rainbow & 4.3$\pm$0.2 & 5.0$\pm$1.3 & 1M \\
      \hline
      SPRING (w/ GPT-4) & 27.3$\pm$1.2 & 12.3$\pm$0.7 & - \\
      Reflexion (w/ GPT-4) & 12.8$\pm$1.0 & 10.3$\pm$1.3 & - \\
      %Reflexion (GPT-4) & 11.7$\pm$1.4 & 9.1$\pm$0.8 & - \\
      ReAct (w/ GPT-4) & 8.3$\pm$1.2 & 7.4$\pm$0.9 & - \\
      Vanilla GPT-4 & 3.4$\pm$1.5 & 2.5$\pm$1.6 & - \\
      \hline
      Human Experts & 50.5$\pm$6.8 & 14.3$\pm$2.3 & - \\
      Random & 1.6$\pm$0.0 & 2.1$\pm$1.3 & - \\
      \hline
    \end{tabular}
    }
    \caption{The results indicate that DLLM with GPT-4 and GPT-3.5 outperforms baseline algorithms, achieving superiority at 1M and 5M training steps.}
    \label{tab:crafter5Mtable_in_main}
    \vspace{-2mm}
  % \end{minipage}%
\end{wraptable}

\textbf{Performance.} DLLM outperforms all baseline algorithms at 1M and 5M steps. As shown in Figure~\ref{fig:crafter_sub_spr} and Table~\ref{tab:crafter5Mtable_in_main}, DLLM exhibits a significant advantage compared to baselines. Figure~\ref{fig:crafter_sub_successes} shows that DLLM is good at medium to high difficulty tasks like ``make stone pickaxe/sword'' and ``collect iron'' while maintaining stable performance in less challenging tasks. When the steps reach 5M, the performance of DLLM significantly surpasses the language-based algorithm SPRING. These findings show strong evidence for hypotheses \textbf{H2} and \textbf{H3}. In all experiments of Crafter, DLLM (w/ GPT-4) demonstrates a more robust performance than DLLM (w/ GPT-3.5), indicating that DLLM can indeed achieve better performance with the assistance of a more powerful LLM. This finding aligns with the results presented in Appendix~\ref{appendix:crafter_goals_analysis}, where GPT-4 consistently identifies exploration-beneficial goals, thus confirming hypothesis \textbf{H4}. In Crafter, We also include ablation studies on the scale of intrinsic rewards in Appendix~\ref{appendix:crafter_ab_scale}, not decreasing intrinsic rewards in Appendix~\ref{appendix:nornd}, utilizing random goals in Appendix~\ref{appendix:randomgoal}, and allowing repeated intrinsic rewards in Appendix~\ref{appendix:notonepertraj}.

\subsection{Minecraft}

\textbf{Environment description.} Several RL environments, e.g., MineRL~\cite{guss2019minerl}, have been constructed based on Minecraft, a popular video game that features a randomly initialized open world with diverse biomes. Minecraft Diamond is a challenging task based on MineRL, with the primary objective of acquiring a diamond. Progressing through the game involves the player collecting resources to craft new items, ensuring his survival, unlocking the technological progress tree, and ultimately achieving the goal of obtaining a diamond within 36000 steps. In Minecraft Diamond, we also have captioners to provide the captions of the observation and transition in natural language form at each step. The environment settings completely mirror those outlined in DreamerV3~\cite{hafner2023mastering}, which includes awarding a +1 reward for each milestone achieved, which encompasses collecting or crafting a log, plank, stick, crafting table, wooden pickaxe, cobblestone, stone pickaxe, iron ore, furnace, iron ingot, iron pickaxe, and diamond.

\begin{table}[ht]
  \begin{minipage}[b]{0.3\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cc}
      \hline
      Method & Reward \\
      \hline
      DLLM (w/ GPT-4) & \textbf{10.0}$\pm$0.3 \\
      DreamerV3 & 9.1$\pm$0.3 \\
      Dynalang & 8.9$\pm$0.4 \\
      IMPALA & 7.4$\pm$0.2 \\
      Rainbow & 6.3$\pm$0.3 \\
      R2D2 & 5.0$\pm$0.5 \\
      PPO & 4.1$\pm$0.2 \\
      ELLM & 0.3$\pm$0.0 \\
      \hline
    \end{tabular}
    }
    \caption{Comparison between DLLM (w/ GPT-4) and baselines in Minecraft at 100M. DLLM (w/ GPT-4) surpasses all baselines, including those that also involve LLMs or natural languages in policy learning.}%with or without the help of natural languages or the LLM.}
    \label{tab:mc_table}
  \end{minipage}\hfill
  \begin{minipage}[b]{0.65\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{icml2024/pics/MC_plot.pdf}
    \captionof{figure}{The episode returns in Minecraft Diamond. The curves indicate that DLLM enjoys a consistent advantage throughout the entire learning process, thanks to its utilization of an LLM for exploration and training. All algorithms undergo experiments using 5 different seeds.}
    \label{mc_plot}
  \end{minipage}
\end{table}

\textbf{Extra baselines.} To fully compare DLLM with current popular methods from model-based algorithms to model-free algorithms on Minecraft, we include DreamerV3~\cite{hafner2023mastering}, IMPALA~\cite{espeholt2018impala}, R2D2~\cite{liu2003r2d2}, Rainbow~\cite{hessel2017rainbow} and PPO~\cite{schulman2017proximal} as our extra baselines, along with ELLM~\cite{du2023guiding} and Dynalang~\cite{lin2023learning}.

\textbf{Query prompts, LLM choices, and Goals Generated.} During each query to the GPT, we provide it with information about the player's status, inventory, and equipment and request the GPT to generate five goals. We choose GPT-4 as our language model for the DLLM experiment. Please see Appendix \ref{appendix:minecrafterprompt} for specific details. We make a query to the GPT every twenty steps. We also test the quality of the generated goals in Appendix~\ref{appendix:mc_goals_analysis}.

\textbf{Performance.} In Figure~\ref{mc_plot} and Table~\ref{tab:mc_table}, we present empirical results in Minecraft Diamond. Baseline algorithm ELLM struggles in this complex environment, possibly due to high task complexity. DLLM demonstrates higher data efficiency in the early training stages, facilitating quicker acquisition of basic skills within fewer training steps compared to baseline methods. DLLM also maintains a significant advantage in later stages, indicating its ability to still derive reasonable and practical guidance from the LLM during the post-exploration training process. These findings underscore the effectiveness of DLLM in guiding exploration and training in highly complex environments with the support of the LLM, providing compelling evidence for hypothesis \textbf{H3}.


% original figure position
% \begin{figure*}[!htb]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.95\textwidth]{icml2024/pics/spectrum-reward.pdf}}
% \vspace{-5mm}
% \caption{Logarithmic scale success rates for unlocking 22 distinct achievements at 1M. DLLM surpasses baselines in the majority of achievements, particularly excelling in challenging tasks such as "make stone pickaxe/sword" and "collect iron."}
% \label{crafter_sqr}
% \end{center}
% \vskip -0.2in
% \end{figure*}

% \begin{table}[ht]
%   \small
%   \centering
%   \caption{The test of goals generated by GPT-3.5 and GPT-4. ``Novel'' represents a goal with its prerequisites completed, but the goal itself still needs to be achieved. `Realistic' signifies that all the conditions for achieving the goal are currently satisfied. ``Meaningless'' indicates a goal that is neither novel nor realistic. ``Unavailable'' denotes a goal that is impossible to accomplish within the game mechanics. Interestingly, we found that GPT-4 tends to provide bold and innovative guidance, while GPT-3.5 is relatively more conservative, leaning towards more practically meaningful guidance.}
%   \begin{tabular}{ccccc}
%     \hline
%     LLM & Novel & Realistic & Meaningless & Unavailable \\
%     \hline
%     GPT-3.5 & 17.44\% & 61.97\% & 20.21\% & 8.26\% \\
%     GPT-4 & 38.15\% & 23.05\% & 38.26\% & 10.78\% \\
%     \hline
%   \end{tabular}
%   \label{tab:crafter_goals}
% \end{table}
% \vspace{-3mm}
% original table position

% \begin{table}[ht]
%   \small
%   \centering
%   \caption{Comparing the performance of DLLM and baselines in terms of score and reward metrics. DLLM experiments utilize 5 different seeds. DLLM outperforms baselines at 1M steps.}
%   \begin{tabular}{cccc}
%     \hline
%     Method & Score & Reward & Steps \\
%     \hline
%     DLLM (w/ GPT4) & 24.88$\pm$8.4\% & 12.0$\pm$1.1 & 1M \\
%     DLLM (w/ GPT3.5) & 23.67$\pm$12.8\% & 12.2$\pm$3.9 & 1M \\
%     RLAdapter (w/ GPT-4) & 15.4$\pm$2.2\% & 12.1$\pm$1.5 & 1M \\
%     RLAdapter (w/ GPT-3.5) & 14.7$\pm$2.3\% & 11.8$\pm$2.1 & 1M \\
%     DreamerV3 & 14.5$\pm$1.6 \% & 11.7$\pm$1.9 & 1M \\
%     PPO & 4.6$\pm$0.3\% & 4.2$\pm$1.2 & 1M \\
%     Rainbow & 4.3$\pm$0.2\% & 5.0$\pm$1.3 & 1M \\
%     Plan2Explore & 2.1$\pm$0.1\% & 2.1$\pm$1.5 & 1M \\
%     RND & 2.0$\pm$0.1 \% & 0.7$\pm$1.3 & 1M \\
%     \hline
%     Human Experts & 50.5$\pm$6.8\% & 14.3$\pm$2.3 & - \\
%     SPRING (w/ GPT-4) & 27.3$\pm$1.2\% & 12.3$\pm$0.7 & - \\
%     GPT-4 & 3.4$\pm$1.5\% & 2.5$\pm$1.6 & - \\
%     Random & 1.6$\pm$0.0\% & 2.1$\pm$1.3 & - \\
%     \hline
%   \end{tabular}
%   \label{tab:crafter_score}
% \end{table}

% \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM exhibits higher mean values but also higher variance. Higher variance arises from some seeds randomly exploring and quickly mastering medium to high-difficulty tasks, while others do not complete this process, leading to significant differences in scores.}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=0.8\columnwidth]{icml2024/pics/homegrid_description.png}}
% \caption{An illustration of the natural language information obtained in different settings in HomeGrid. Standard, key info and full info share the existing information in the field of view. Key info additionally acquires task-related information, while full info obtains all the information on the map.}
% \label{homegrid_des}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \lzy{\sout{To testify our hyphothsis, we developed three criterias: the level of commonsense knowledge gained by lanugage model, the scale of novlety of the actions LMs proposes, also the proportion of unavailable tasks LMs generated. (detailed explaination, have little idea about how to explain them).
% (A1): Commonsense knowlegde
% (A2): Novelty
% (A3): Unavailable.}}
% \lzy{The primary goal of our experiments is to substantiate the following claim: DLLM helps the agent consider guidance from the large language model during the dreaming process, thereby achieving improved performance in tasks. We test four specific hypotheses:}
% \lzy{\sout{The primary goal of our experiments is to substantiate the following claim: DLLM helps the agent consider guidance from the large language model during the dreaming process, thereby achieving improved performance in tasks. We compare DLLM with other baseline algorithms in environments such as HomeGrid, Crafter, and Minecraft to substantiate this point. We also examine whether the agent's performance improves by gradually providing more information to the LLM or by utilizing a relatively more powerful LLM.}}\\
% \ziyu{
% \sout{DLLM helps the agent consider guidance from the large language model during the dreaming process, thereby achieving improved performance in tasks. We compare DLLM with other baseline algorithms in environments such as HomeGrid, Crafter, and Minecraft to substantiate this point. Our experiments substantiates the following questions (hypotheses):}}\\
% \ziyu{\sout{(H1): Pretrained Large Language Models can understand embodied environment through its commonsense knowledge, thus using these knowledge to help guide agents towards various goals and task completion. This would also avoid the situation where the agent have to learn through exploration and failure. To test this, we involve HomeGrid environment where the agent have to understand the environment towards task completion.
% (H2): Whether DLLM(Language guided MBRL) can efficiently help the exploration
% (H3):Whether the approach of combining language priors with world models could assist multi-step planning, thus even adds up to solve super complex tasks}}\\
% \ziyu{\sout{To testify our hyphothsis, we developed three criterias: the level of commonsense knowledge gained by lanugage model, the scale of novlety of the actions LMs proposes, also the proportion of unavailable tasks LMs generated. (detailed explaination, have little idea about how to explain them).
% (A1): Commonsense knowlegde
% (A2): Novelty
% (A3): Unavailable}}
% \sout{DLLM helps the agent consider guidance from the large language model during the dreaming process, thereby achieving improved performance in tasks.
% \item \textbf{(H2)} Through purposeful prompting, DLLM can assit agents in various types of tasks, including task completion, exploration, or highly complex, realistic integrated tasks.
% \item \textbf{(H3)} DLLM naturally enhances its performance when leveraging stronger LLMs or receiving additional language information.}

% \begin{itemize}
%   \item \textbf{Standard.} The environment provides only task descriptions and descriptions of each step's transition.
%   \item \textbf{Key info.} The environment additionally provides task-relevant objects' location and status information.
%   \item \textbf{Full info.} The environment additionally provides the location and status information of all objects on the map. For bins, the correct opening actions will also be instructed.
%   \item \textbf{Oracle.} The agent will always receive accurate instructions.
% \end{itemize}

% \lzy{\sout{\textbf{Baselines.} Due to the fact that there exist natural language information in the observation space of HomeGrid and many previous baseline methods do not involve languages as inputs, we specifically choose ELLM~\cite{du2023guiding} and Dynalang~\cite{lin2023learning} as our baselines. We use identical language observations for all algorithms. For ELLM, we prompt the LLM and obtain goals following the same procedure as in our method. Since Dynalang utilizes a token-by-token method to tokenize task descriptions in its experiments, we conducted relevant experiments in the ablation study (Appendix~\ref{appendix:dynalangtoken}). However, no significant differences in performance were observed.}}
%Due to the presence of natural language in the observation space of HomeGrid, we specifically chose baseline algorithms that can leverage natural language. We compare with model-free RL baselines ELLM~\cite{du2023guiding} and the model-based RL baseline Dynalang~\cite{lin2023learning}. We provide the same language observations to the baselines as to our method. Due to Dynalang utilizing a token-by-token method to tokenize task descriptions in its experiments, we conducted relevant experiments in the ablation study~\ref{appendix:dynalangtoken}. However, no significant differences in performance were observed.

%We made the following modifications to the original environment: Firstly, ..., Secondly, we set up the environment to articulate the transitions the agent undertook at each time step, expressed in natural language (e.g., ``go to the kitchen'', ``pick up the fruits''). 

% \noindent \textbf{Standard.} The environment provides only task descriptions.

% \noindent\textbf{Key info.} The environment additionally provides task-relevant objects' location and status information.

% \noindent\textbf{Full info.} The environment additionally provides the location and status information of all objects on the map. For bins, the correct opening actions will also be instructed.

% \noindent\textbf{Oracle.} The agent will always receive accurate instructions.

% \caption{Testing the accuracy of goals provided by LLM in each setting. The accuracy in both aspects is low in the standard setting since the agent's observation may lack relevant information. There is a noticeable improvement in the key info part. The full info part has an additional improvement in the ``what to do'' aspect, as we provide instructions for the correct opening actions for each bin.}
%We observe that our method outperforms various baselines across all experimental designs. For DLLM, the experiments with key info and full info show a more pronounced advantage compared to the standard experiment. We believe this demonstrates that the introduction of more precise goals by LLM indeed contributes to the performance improvement of the DLLM agent. Regarding key info and full info, we observe no significant difference between the experimental results. Each experiment was conducted with 5 different seeds.

% \begin{table}[ht]
% %\begin{wraptable}{r}{0.66\textwidth}
%   \small
%   \centering
%   \caption{Performance comparison of DLLM and baselines in terms of score and reward metrics. DLLM experiments utilize 5 different seeds. DLLM outperforms baselines at 1M steps.}
%   \begin{tabular}{cccc}
%     \hline
%     Method & Score & Reward & Steps \\
%     \hline
%     DLLM (w/ GPT4) & \textbf{24.9}$\pm$0.8\% & 12.0$\pm$1.1 & 1M \\
%     DLLM (w/ GPT3.5) & \textbf{23.7}$\pm$1.3\% & 12.2$\pm$3.9 & 1M \\
%     Achievement Distillation \cite{moon2024discovering}& 21.8$\pm$1.4\% & 12.6$\pm$0.3 & 1M \\
%     AdaRefiner (w/ GPT-4) & 15.8$\pm$1.4\% & 12.3$\pm$1.3 & 1M \\
%     PPO (tuned) & 15.6$\pm$1.7\% & 10.3$\pm$0.5 & 1M \\
%     DreamerV3 & 14.5$\pm$1.6 \% & 11.7$\pm$1.9 & 1M \\
%     PPO & 4.6$\pm$0.3\% & 4.2$\pm$1.2 & 1M \\
%     Rainbow & 4.3$\pm$0.2\% & 5.0$\pm$1.3 & 1M \\
%     Plan2Explore & 2.1$\pm$0.1\% & 2.1$\pm$1.5 & 1M \\
%     RND & 2.0$\pm$0.1 \% & 0.7$\pm$1.3 & 1M \\
%     \hline
%     Human Experts & 50.5$\pm$6.8\% & 14.3$\pm$2.3 & - \\
%     SPRING (w/ GPT-4) & 27.3$\pm$1.2\% & 12.3$\pm$0.7 & - \\
%     GPT-4 & 3.4$\pm$1.5\% & 2.5$\pm$1.6 & - \\
%     Random & 1.6$\pm$0.0\% & 2.1$\pm$1.3 & - \\
%     \hline
%   \end{tabular}
%   \label{tab:crafter_score}
% \end{table}
% %\end{wraptable}

% We modify the original Crafter to articulate the transitions undertaken by the agent at each time step in the form of natural language (e.g., ``make wooden pickaxe'', ``attack zombie''). For more details, please check \ref{appendix:crafterenvmod}.

% \begin{figure}[!htb]
% \centering
% \begin{subfigure}
%   \centering
%   \includegraphics[width=0.3\textwidth]{icml2024/pics/scores-agents.pdf}
%   % \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin. DLLM with GPT-3.5 tends to have a higher variance in its performance, possibly due to the instability in GPT-3.5 (e.g., generated goals are unstable).}
%   \label{fig:subfig1}
% \end{subfigure}
% \hfill
% \begin{subfigure}
%   \centering
%   \includegraphics[width=0.65\textwidth]{icml2024/pics/spectrum-reward.pdf}
%   \label{fig:subfig2}
% \caption{(a): Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin. DLLM with GPT-3.5 tends to have a higher variance in its performance, possibly due to the instability in GPT-3.5 (e.g., generated goals are unstable). (b): Logarithmic scale success rates for unlocking 22 distinct achievements at 1M. DLLM surpasses baselines in the majority of achievements, particularly excelling in challenging tasks such as ``make stone pickaxe/sword" and ``collect iron."}
% \end{subfigure}
% %\caption{Comparison of DLLM with baselines}
% %\label{fig:double_figures}
% \end{figure}

% \begin{figure}[!htb]
%   \centering
%   \begin{subfigure}{0.3\textwidth}
%     \centering
%     \begin{tabular}{cccc}
%       \hline
%       Method & Score & Reward & Steps \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{38.1}$\pm$1.2 & 15.4$\pm$1.1 & 5M \\
%       DLLM (w/ GPT3.5) & \textbf{37.6}$\pm$1.6 & 14.5$\pm$1.5 & 5M \\
%       AdaRefiner (w/ GPT4) & 28.2$\pm$1.8 & 12.9$\pm$1.2 & 5M \\
%       AdaRefiner (w/ GPT-3.5) & 23.4$\pm$2.2 & 11.8$\pm$1.7 & 5M \\
%       ELLM & - & 6.0$\pm$0.4 & 5M \\
%       \hline
%       Human Experts & 50.5$\pm$6.8\% & 14.3$\pm$2.3 & - \\
%       SPRING (w/ GPT-4) & 27.3$\pm$1.2\% & 12.3$\pm$0.7 & - \\
%       GPT-4 & 3.4$\pm$1.5\% & 2.5$\pm$1.6 & - \\
%       Random & 1.6$\pm$0.0\% & 2.1$\pm$1.3 & - \\
%       \hline
%     \end{tabular}
%     \caption{The results of 5M in Crafter. DLLM outperforms all baselines.}
%     \label{tab:crafter5Mtable}
%   \end{subfigure}%
  
%   \begin{subfigure}{0.3\textwidth}
%     \centering
%     \begin{tabular}{ccc}
%       \hline
%       Col1 & Col2 & Col3 \\
%       \hline
%       1 & 2 & 3 \\
%       4 & 5 & 6 \\
%       7 & 8 & 9 \\
%       \hline
%     \end{tabular}
%     \caption{Another table}
%     \label{tab:anothertable}
%   \end{subfigure}
%   \begin{subfigure}{0.3\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{example-image-a}
%     \caption{Your figure}
%     \label{fig:yourfigure}
%   \end{subfigure}
%   \caption{Overall caption}
%   \label{fig:overall}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
% \centering
% \includegraphics[width=0.43\textwidth]{icml2024/pics/spr_overall.pdf}
% \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin.}
% \label{crafter_bar}

% \begin{figure*}[!htb]
% \centering
% \includegraphics[width=\textwidth]{icml2024/pics/spectrum-reward.pdf}
% \caption{Logarithmic scale success rates for unlocking 22 distinct achievements at 1M. DLLM surpasses baselines in most achievements, particularly excelling in challenging tasks such as ``make stone pickaxe/sword" and ``collect iron."}
% \label{crafter_sqr}
% \end{figure*}

% \begin{table}[ht]
% %\begin{wraptable}{r}{0.66\textwidth}
%   \small
%   \centering
%   \caption{Performance comparison of DLLM and baselines in terms of score and reward metrics. DLLM experiments utilize 5 different seeds. DLLM outperforms baselines at 1M steps.}
%   \begin{tabular}{cccc}
%     \hline
%     Method & Score & Reward & Steps \\
%     \hline
%     DLLM (w/ GPT4) & \textbf{26.4}$\pm$1.3 & 12.4$\pm$1.3 & 1M \\
%     DLLM (w/ GPT3.5) & \textbf{24.4}$\pm$1.8 & 12.2$\pm$1.6 & 1M \\
%     Achievement Distillation~\cite{moon2024discovering}& 21.8$\pm$1.4 & 12.6$\pm$0.3 & 1M \\
%     DLLM (random goal) & 19.2$\pm$1.1 & 11.3$\pm$0.3 & 1M \\
%     DLLM (not one per traj) & 17.1$\pm$1.5 & 10.9$\pm$3.0 & 1M \\
%     Dynalang & 16.4$\pm$1.7 & 10.5$\pm$1.4 & 1M \\
%     AdaRefiner (w/ GPT-4) & 15.8$\pm$1.4 & 12.3$\pm$1.3 & 1M \\
%     PPO (ResNet) & 15.6$\pm$1.6 & 10.3$\pm$0.5 & 1M \\
%     DreamerV3 & 14.5$\pm$1.6 & 11.7$\pm$1.9 & 1M \\
%     DLLM (no decrease) & 14.3$\pm$2.3 & 10.5$\pm$2.1 & 1M \\
%     PPO & 4.6$\pm$0.3 & 4.2$\pm$1.2 & 1M \\
%     Rainbow & 4.3$\pm$0.2 & 5.0$\pm$1.3 & 1M \\
%     \hline
%     Human Experts & 50.5$\pm$6.8 & 14.3$\pm$2.3 & - \\
%     SPRING (w/ GPT-4) & 27.3$\pm$1.2 & 12.3$\pm$0.7 & - \\
%     GPT-4 & 3.4$\pm$1.5 & 2.5$\pm$1.6 & - \\
%     Random & 1.6$\pm$0.0 & 2.1$\pm$1.3 & - \\
%     \hline
%   \end{tabular}
%   \label{tab:crafter_score}
% \end{table}
%\end{wraptable}

% Figure \ref{crafter_sqr5M} and Table \ref{tab:crafter5Mtable} present the performance comparison between DLLM and other baselines in Crafter at 5M steps. DLLM exhibits a higher success rate in unlocking fundamental achievements and outperforms other baselines regarding overall scores.
% \begin{figure}[!htb]
%   \centering
%   \begin{subfigure}{0.3\textwidth}
%     \centering
%     \begin{tabular}{cccc}
%       \hline
%       Method & Score & Reward & Steps \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{38.1}$\pm$1.2 & 15.4$\pm$1.1 & 5M \\
%       DLLM (w/ GPT3.5) & \textbf{37.6}$\pm$1.6 & 14.5$\pm$1.5 & 5M \\
%       AdaRefiner (w/ GPT4) & 28.2$\pm$1.8 & 12.9$\pm$1.2 & 5M \\
%       AdaRefiner (w/ GPT-3.5) & 23.4$\pm$2.2 & 11.8$\pm$1.7 & 5M \\
%       ELLM & - & 6.0$\pm$0.4 & 5M \\
%       \hline
%       Human Experts & 50.5$\pm$6.8\% & 14.3$\pm$2.3 & - \\
%       SPRING (w/ GPT-4) & 27.3$\pm$1.2\% & 12.3$\pm$0.7 & - \\
%       GPT-4 & 3.4$\pm$1.5\% & 2.5$\pm$1.6 & - \\
%       Random & 1.6$\pm$0.0\% & 2.1$\pm$1.3 & - \\
%       \hline
%     \end{tabular}
%     \caption{Table 1}
%     \label{tab:crafter5Mtable}
%   \end{subfigure}%
%   \begin{subfigure}{0.3\textwidth}
%     \centering
%     \begin{tabular}{cccc}
%       \hline
%       Method & Score & Reward & Steps \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{26.4}$\pm$1.3 & 12.4$\pm$1.3 & 1M \\
%       DLLM (w/ GPT3.5) & \textbf{24.4}$\pm$1.8 & 12.2$\pm$1.6 & 1M \\
%       Achievement Distillation~\cite{moon2024discovering}& 21.8$\pm$1.4 & 12.6$\pm$0.3 & 1M \\
%       DLLM (random goal) & 19.2$\pm$1.1 & 11.3$\pm$0.3 & 1M \\
%       DLLM (not one per traj) & 17.1$\pm$1.5 & 10.9$\pm$3.0 & 1M \\
%       Dynalang & 16.4$\pm$1.7 & 10.5$\pm$1.4 & 1M \\
%       AdaRefiner (w/ GPT-4) & 15.8$\pm$1.4 & 12.3$\pm$1.3 & 1M \\
%       PPO (ResNet) & 15.6$\pm$1.6 & 10.3$\pm$0.5 & 1M \\
%       DreamerV3 & 14.5$\pm$1.6 & 11.7$\pm$1.9 & 1M \\
%       DLLM (no decrease) & 14.3$\pm$2.3 & 10.5$\pm$2.1 & 1M \\
%       PPO & 4.6$\pm$0.3 & 4.2$\pm$1.2 & 1M \\
%       Rainbow & 4.3$\pm$0.2 & 5.0$\pm$1.3 & 1M \\
%       \hline
%       Human Experts & 50.5$\pm$6.8 & 14.3$\pm$2.3 & - \\
%       SPRING (w/ GPT-4) & 27.3$\pm$1.2 & 12.3$\pm$0.7 & - \\
%       GPT-4 & 3.4$\pm$1.5 & 2.5$\pm$1.6 & - \\
%       Random & 1.6$\pm$0.0 & 2.1$\pm$1.3 & - \\
%       \hline
%     \end{tabular}
%     \caption{Table 2}
%     \label{tab:crafter_score}
%   \end{subfigure}
  
%      \begin{subfigure}{0.3\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{icml2024/pics/MCreward.pdf}
%         \caption{\lzy{\sout{The episode returns to the Minecraft environment. The graph shows that DLLM exhibits an early advantage due to leveraging a large language model for exploration assistance. Both DLLM and DreamerV3 undergo experiments using 3 different seeds.}}}
%         \label{minecraft_plot}
%       \end{subfigure}
%       \caption{Overall caption}
%       \label{fig:overall}
%     \end{figure}

% \begin{figure}[ht]
% \centering
%     \begin{subfigure}{0.37\linewidth}
%     \centering
%     \includegraphics[width=0.3\linewidth]{icml2024/pics/spr_overall.pdf}
%     \captionsetup{labelformat=empty} % 设置子图标号不显示
%     \caption{(a)} % 手动设置子图标号
%     \end{subfigure}
%     \begin{subfigure}{0.60\linewidth}
%     \centering
%     \includegraphics[width=0.5\linewidth]{icml2024/pics/successes.png}
%     \captionsetup{labelformat=empty} % 设置子图标号不显示
%     \caption{(b)} % 手动设置子图标号
%     \end{subfigure}
% \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin. Logarithmic scale success rates for unlocking 22 distinct achievements at 1M. DLLM surpasses baselines in most achievements, particularly excelling in challenging tasks such as ``make stone pickaxe/sword" and ``collect iron."}
% \label{crafter_sqr}
% \end{figure}

% \begin{wrapfigure}{r}{0.5\textwidth}
% \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin.}
%\label{crafter_bar}


% \begin{wrapfigure}{r}{0.47\textwidth}
% \begin{center}
% \centerline{\includegraphics[width=0.65\textwidth]{icml2024/pics/MC_plot.pdf}}
% \caption{The episode returns to the Minecraft environment. The graph indicates that DLLM enjoys a consistent advantage throughout the entire episode, attributed to its utilization of a large language model for exploration and training. All algorithms undergo experiments using 5 different seeds.}
% \label{minecraft_plot}
% \end{center}
% \end{wrapfigure}

% \begin{wraptable}{r}{0.5\textwidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{cc|cc}
%       \hline
%       Method & Reward & Method & Reward \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{10.0}$\pm$0.3 & Rainbow & 6.3$\pm$0.3 \\
%       DreamerV3 & 9.1$\pm$0.3 & PPO & 4.1$\pm$0.2 \\
%       Dynalang & 8.9$\pm$0.4 & R2D2 & 5.0$\pm$0.5 \\
%       IMPALA & 7.4$\pm$0.2 & ELLM & 0.3$\pm$0.0 \\
%       \hline
%     \end{tabular}
%     }
%     \caption{\lzy{Complete it.}}
%     \label{tab:MCtable}
% \end{wraptable}

% \begin{wraptable}{r}{0.33\textwidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{cc}
%       \hline
%       Method & Reward \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{10.0}$\pm$0.3 \\
%       DreamerV3 & 9.1$\pm$0.3 \\
%       Dynalang & 8.9$\pm$0.4 \\
%       IMPALA & 7.4$\pm$0.2 \\
%       Rainbow & 6.3$\pm$0.3 \\
%       PPO & 4.1$\pm$0.2 \\
%       R2D2 & 5.0$\pm$0.5 \\
%       ELLM & 0.3$\pm$0.0 \\
%       \hline
%     \end{tabular}
%     }
%     \caption{\lzy{Complete it.}}
%     \label{tab:MCtable}
% \end{wraptable}

% \begin{table}[ht]
%   \begin{minipage}[t]{0.33\linewidth}
%     \centering
%     \resizebox{\linewidth}{!}{%
%     \begin{tabular}{cc}
%       \hline
%       Method & Reward \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{10.0}$\pm$0.3 \\
%       DreamerV3 & 9.1$\pm$0.3 \\
%       Dynalang & 8.9$\pm$0.4 \\
%       IMPALA & 7.4$\pm$0.2 \\
%       Rainbow & 6.3$\pm$0.3 \\
%       PPO & 4.1$\pm$0.2 \\
%       R2D2 & 5.0$\pm$0.5 \\
%       ELLM & 0.3$\pm$0.0 \\
%       \hline
%     \end{tabular}
%     }
%     \caption{Table caption}
%     \label{tab:crafter5Mtable}
%   \end{minipage}\hfill
%   \begin{minipage}[t]{0.7\linewidth}
%     \centering
%     \includegraphics[width=0.8\linewidth]{icml2024/pics/MC_plot.pdf}
%     \captionof{figure}{Figure caption}
%     \label{fig:mcplot}
%   \end{minipage}
% \end{table}

%\textbf{Captioner and Language Encodings.} For each environment, we have an observation captioner and a transition captioner to caption the observations and transitions. The captions of transitions are stored in the dataset for the agent's learning to predict, and the captions describing the observations are used to provide related information for LLM. For language encoding, we use SentenceBert \emph{all-MiniLM-L6-v2}~\cite{wang2020minilm} to convert all these natural information into embeddings. %; please see appendix~\ref{appendix:captioner} for more details~\lzy{}

% \caption{Bar chart comparison of the means and variances between DLLM and baselines. DLLM generally exhibits higher average performance, surpassing baselines by a large margin.}

% \begin{table}[ht]
%   \begin{minipage}[b]{0.3\linewidth}
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cc}
%       \hline
%       Method & Reward \\
%       \hline
%       DLLM (w/ GPT4) & \textbf{10.0}$\pm$0.3 \\
%       DreamerV3 & 9.1$\pm$0.3 \\
%       Dynalang & 8.9$\pm$0.4 \\
%       IMPALA & 7.4$\pm$0.2 \\
%       Rainbow & 6.3$\pm$0.3 \\
%       R2D2 & 5.0$\pm$0.5 \\
%       PPO & 4.1$\pm$0.2 \\
%       ELLM & 0.3$\pm$0.0 \\
%       \hline
%     \end{tabular}
%     }
%     \caption{Comparison between DLLM (w/ GPT4) and baselines in Minecraft at 100M.\lzy{Need to split these two.}}
%     \label{tab:mc_table}
%   \end{minipage}\hfill
% \begin{subfigure}%{0.3\textwidth}
%     \centering
%     \includegraphics[width=0.66\textwidth]{icml2024/pics/MC_plot.pdf}
%     \captionof{figure}{The episode returns to the Minecraft environment. The graph indicates that DLLM enjoys a consistent advantage throughout the entire episode, attributed to its utilization of a large language model for exploration and training. All algorithms undergo experiments using 5 different seeds.}
%     \label{mc_plot}
% \end{subfigure}
% \end{table}

%The Crafter environment is a procedurally generated open-world survival game for benchmarking RL algorithms.

% (see Appendix \ref{appendix:5Mcrafter} for the results), 

% \sout{Minecraft is a popular video game that features a randomly initialized open world with diverse biomes. The world is constructed using 1-meter-sized blocks, allowing players to break, place, or interact with them. Additionally, approximately 30 different types of creatures are present in this dynamic environment. The primary objective in Minecraft Diamond is to acquire diamonds, a goal akin to that in the Crafter environment but with heightened difficulty. Progressing through the game involves players collecting resources to craft new items, ensuring their safety and survival, unlocking the technological progress tree, and ultimately achieving the goal of obtaining diamonds. We also have the captioners to provide the captions of the observation and transitions in natural language form at each step. The environment settings completely mirror those outlined in DreamerV3~\cite{hafner2023mastering}, which includes awarding a +1 reward for each milestone achieved, which encompasses collecting logs, planks, sticks, crafting tables, wooden pickaxes, cobblestones, stone pickaxes, iron ores, furnaces, iron ingots, iron pickaxes, and diamonds.}


% \begin{table}[ht]
% \centering
% \caption{Description of different environment settings}
% \begin{tabular}{lp{11.8cm}}
% \hline
% \textbf{Setting} & \textbf{Description} \\
% \hline
% Standard & The environment provides task descriptions in natural language form. \\
% \hline
% Key info & The environment additionally provides task-relevant objects' location and status information. \\
% \hline
% Full info & The environment additionally provides the location and status information of all objects on the map. For bins, the correct opening actions will also be instructed. \\
% \hline
% Oracle & The agent will always receive accurate instructions. \\
% \hline
% \end{tabular}
% \label{tab:environment_settings}
% \end{table}

%naturally enhances its performance when leveraging stronger large language models or receiving additional language information.

==> icml2024/6_conclusion.tex <==
\section{Conclusion and Discussion}

We propose DLLM, a multi-modal model-based RL method that leverages the guidance from LLMs to provide hints (goals) and generate intrinsic rewards in model rollouts. DLLM outperforms recent strong baselines in multiple challenging tasks with sparse rewards. Our experiments demonstrate that DLLM effectively utilizes language information from the environment and LLMs, and enhances its performance by improving language information quality.

\textbf{Limitations.} DLLM relies on the guidance provided by a large language model, making it susceptible to the inherent instability of LLM outputs. This introduces a potential risk to the stability of DLLM's performance, even though the prompts used in our experiments contributed to relatively stable model outputs. Unreasonable goals may encourage the agent to make erroneous attempts, and correcting such misguided behavior may take time. We expect to address these challenges in future work.

%\textbf{Limitations.} 

% \section{Impact statements}
% LLMs have the potential to produce harmful or biased information. We have not observed LLMs generating such content in our current experimental environments, including HomeGrid, Crafter, and Minecraft. However, applying DLLM in other contexts, especially real-world settings, requires increased attention to social safety concerns. Implementing necessary safety measures involves screening LLM outputs, incorporating restrictive statements in LLM prompts, or fine-tuning with curated data.

%Conclusion and Discussion
